Reinforcement Learning for Unified Allocation and Patrolling in Signaling Games with Uncertainty

Green Security Games (GSGs) have been successfully used in the protection of valuable resources such as fisheries, forests and wildlife. While real-world deployment involves both resource allocation and subsequent coordinated patrolling with communication and real-time, uncertain information, previous game models do not fully address both of these stages simultaneously. Furthermore, adopting existing solution strategies is difficult since they do not scale well for larger, more complex variants of the game models. We therefore first propose a novel GSG model that combines defender allocation, patrolling, real-time drone notification to human patrollers, and drones sending warning signals to attackers. The model further incorporates uncertainty for real-time decision-making within a team of drones and human patrollers. Second, we present CombSGPO, a novel and scalable algorithm based on reinforcement learning, to compute a defender strategy for this game model. CombSGPO performs policy search over a multi-dimensional, discrete action space to compute an allocation strategy that is best suited to a best-response patrolling strategy for the defender, learnt by training a multi-agent Deep Q-Network. We show via experiments that CombSGPO converges to better strategies and is more scalable than comparable approaches. Third, we provide a detailed analysis of the coordination and signaling behavior learnt by CombSGPO, showing group formation between defender resources and patrolling formations based on signaling and notifications between resources. Importantly, we find that strategic signaling emerges in the final learnt strategy. Finally, we perform experiments to evaluate these strategies under different levels of uncertainty.

==> not_required.tex <==
\section{Neural Network Architecture}

We first describe the neural network architecture for DQNs used in the patrolling stage of the games. We then describe the neural networks that were used to represent allocation strategies for the defender and the attacker.

The DQN had two convolution layers with the non-linear \texit{ReLU} activations between them. The first convolutional layer had 10 filters of size 3x3 and strides 1x1 while the second convolutional layer had 20 filters of size 3x3 and strides 1x1. The convolutional layers were followed by two fully-connected dense layers with 128 hidden units and 64 hidden units, respectively, with \texit{ReLU} activations in between. The last layer was a fully-connected dense layer with 5 units representing the 5 actions for the ranger DQN and 15 units representing the actions for the drone DQN.

Allocation strategies were represented by an actor network and a critic network. The actor network had a single fully-connected layer with a non-linear \textit{tanh} activation connected to two layers; the first being a linear layer followed by a \textit{tanh} activation for predicting the mean of the action embedding distribution and the second, a linear layer followed by a \textit{sigmoid} activation for predicting the variance of the action embedding distribution. The critic network had a fully-connected layer with \textit{tanh} activation followed by layer with a single unit for predicting the reward from choosing an allocation. Table 1 details the action embedding sizes used and Table 2 details the number of hidden units used in each layer for the networks described above.

\begin{table}[h]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
Gridsize           & \#Poachers & Defender & Attacker           \\ \hline
\multirow{2}{*}{15x15}  & 1          & 50 & 2 \\ \cline{2-4} 
                         & 2          & 50 & 4 \\ \hline
\multirow{2}{*}{10x10} & 1          & 30 & 2 \\ \cline{2-4} 
                         & 2          & 30 & 4 \\ \hline
\end{tabular}
\caption{Action embedding sizes}
\label{tab:results1}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
Gridsize           & \#Poachers & Defender & Attacker           \\ \hline
\multirow{2}{*}{15x15}  & 1          & 128 & 128 \\ \cline{2-4} 
                         & 2          & 32 & 128 \\ \hline
\multirow{2}{*}{10x10} & 1          & 64 & 32 \\ \cline{2-4} 
                         & 2          & 32 & 32 \\ \hline
\end{tabular}
\caption{Neural Network Architectures : Allocation Policies}
\label{tab:results1}
\end{table}


\section{Neural Network Training}

Tables 3 and 4 show the parameters used while training the ranger and drone DQNs, respectively, for different grid sizes. The DQNs follow an $\epsilon$ greedy policy and during training, $\epsilon$ = 1.0 initially and decays to 0.05 within 25000 steps. A discounting factor of 0.99 is used for calculating the discounted rewards for DQN training. For training, we use the Adam optimizer with $\beta1$ = 0.9 and $\beta2$ = 0.999.

While training the allocation policies, we use the Adam optimizer for updating the critic network, setting the critic learning rate at 1e-2 for both players. We use a batch size of 10 for all of these experiments. Tables 5 shows the learning rates for competitive policy optimization, for experiments with different grid sizes and animal density distributions.
\newpage


\section{Animal Densities}

We perform experiments with two different kinds of animal densities : randomly distributed and spatially distributed. Here, we describe how we calculate spatially distributed animal densities. This distribution reflects the attractiveness of each cell in the park to a potential poacher. We assume that the distribution of targets that are of interest to poachers, is influenced by certain geographical and man-made features; namely : rivers, boundaries of the national park and roads (some of these features are used in (Gholami et al. 2018) to model poacher behavior). 

We consider boundaries at all edges of the grid and we also consider that a river and a road pass through the national park. We then rank each cell depending on it's distance from these features such that cells farther away have a higher rank, as shown in Fig. 4. We then take a weighted average of these ranks to get a measure of how attract a cell is to animals, with weights of 0.1, 0,1 and 0.8 given to the boundary, road and river ranks respectively and call it the animal rank. By further taking a weighted average of animal, river, road and boundary ranks with weights of 0.7, 0.05, 0.15 and 0.1, we arrive at the final animal density distribution.


\begin{table}[h]
\centering
\begin{tabular}{|l|l|l|} \hline
 
 Hyperparameter & 15x15 & 10x10 \\  \hline

 Learning rate & 3e-4 & 3e-4\\ \hline
 Replay Buffer size & 1.92e-5   & 1.92e-4 \\ \hline
 Batch size & 32  & 32\\ \hline
 Target update step & 20 & 20\\\hline
 
 \hline
\end{tabular}
\caption{Parameters for Training : Drone DQN}
\label{table:2}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{|l|l|l|} \hline
 
 Hyperparameter & 15x15 & 10x10 \\  \hline

 Learning rate & 3e-4 & 3e-4\\ \hline
 Replay Buffer size & 0.64e-5   & 0.64e-4 \\ \hline
 Batch size & 32  & 32\\ \hline
 Target update step & 50 & 50\\\hline
 
 \hline
\end{tabular}
\caption{Parameters for Training : Ranger DQN}
\label{table:2}
\end{table}


\begin{table}[h]
\centering
\begin{tabular}{|l|l|l|}
\hline
Gridsize           & \#Poachers & Learning rate      \\ \hline
\multirow{2}{*}{15x15}  & 1           & 4e-5 \\ \cline{2-3} 
                         & 2          & 3e-5 \\ \hline
\multirow{2}{*}{10x10} & 1          & 3e-5 \\ \cline{2-3} 
                         & 2          & 3e-5 \\ \hline
\end{tabular}
\caption{Learning Rates : Allocation Policies}
\label{tab:results1}
\end{table}

\begin{figure*}[h]
\centering
\includegraphics[width=140mm]{Images/adcollage.jpg}
\caption{Left to Right : Ranking of cells based on a. distance from river, b. distance from road and c. distance from boundaries for a 15x15 grid} 
\end{figure*}
\section{Additional Experiments}
\section{Signalling Behavior}

\section{Other learning curves}
We show the learning curves for all baselines and coPG under different uncertainty conditions in figures \ref{fig:coPGall}, \ref{fig:optgradall} and \ref{fig:guardssall}.
\begin{figure}[h]
    \centering
    \begin{subfigure}{.5\linewidth}
      \centering
      \includegraphics[width=\linewidth]{Images/single_random_CoPG_UC.png}
    \end{subfigure}%
    \begin{subfigure}{.5\linewidth}
      \centering
      \includegraphics[width=\linewidth]{Images/single_spatial_coPG_UC.png}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
      \centering
      \includegraphics[width=\linewidth]{Images/multi_random_coPG_UC.png}
    \end{subfigure}%
    \begin{subfigure}{.5\linewidth}
      \centering
      \includegraphics[width=\linewidth]{Images/multi_spatial_coPG_UC.png}
    \end{subfigure}
   \caption{Training reward curves for coPG with different uncertainities}
   \label{fig:coPGall}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}{.5\linewidth}
      \centering
      \includegraphics[width=\linewidth]{Images/single_random_optgrad_UC.png}
    \end{subfigure}%
    \begin{subfigure}{.5\linewidth}
      \centering
      \includegraphics[width=\linewidth]{Images/single_spatial_optgrad_UC.png}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
      \centering
      \includegraphics[width=\linewidth]{Images/multi_random_optgrad_UC.png}
    \end{subfigure}%
    \begin{subfigure}{.5\linewidth}
      \centering
      \includegraphics[width=\linewidth]{Images/multi_spatial_optgrad_UC.png}
    \end{subfigure}
   \caption{Training reward curves for OPTGradFP with different uncertainities}
   \label{fig:optgradall}
\end{figure}


\begin{figure}[h]
    \centering
    \begin{subfigure}{.5\linewidth}
      \centering
      \includegraphics[width=\linewidth]{Images/single_random_GUARDSS_UC.png}
    \end{subfigure}%
    \begin{subfigure}{.5\linewidth}
      \centering
      \includegraphics[width=\linewidth]{Images/single_spatial_GUARDSS_UC.png}
    \end{subfigure}
   \caption{Training reward curves for GUARDSS with different uncertainities}
   \label{fig:guardssall}
\end{figure}

